Wyner-Ziv Estimators for Distributed Mean Estimation with Side Information and Optimization

Communication efficient distributed mean estimation is an important primitive that arises in many distributed learning and optimization scenarios such as federated learning. Without any probabilistic assumptions on the underlying data, we study the problem of distributed mean estimation where the server has access to side information. We propose \emph{Wyner-Ziv estimators}, which are communication and computationally efficient and near-optimal when an upper bound for the distance between the side information and the data is known. As a corollary, we also show that our algorithms provide efficient schemes for the classic Wyner-Ziv problem in information theory. In a different direction, when there is no knowledge assumed about the distance between side information and the data, we present an alternative Wyner-Ziv estimator that uses correlated sampling. This latter setting offers {\em universal recovery guarantees}, and perhaps will be of interest in practice when the number of users is large and keeping track of the distances between the data and the side information may not be possible. With this mean estimator at our disposal, we revisit basic problems in decentralized optimization and compression where our Wyner-Ziv estimator yields algorithms with almost optimal performance. First, we consider the problem of communication constrained distributed optimization and provide an algorithm which attains the optimal convergence rate by exploiting the fact that the gradient estimates are close to each other. Specifically, the gradient compression scheme in our algorithm first uses half of the parties to form side information and then uses our Wyner-Ziv estimator to compress the remaining half of the gradient estimates.

==> setup.tex <==
\section{Application: Distributed optimization} \label{s:setup}
We consider the
problem of minimizing an unknown convex function ${f\colon\X
\to \R}$ over its domain ${\X\subset \R^d}$ 
using a set of $K$ \emph{clients} who have access
to independent noisy gradients of the
function.
In particular, the optimization algorithm is not directly given access to the function
but can get $K$ different gradient estimates of the function at various points of its choice.
This class of optimization algorithms includes various descent algorithms,
which provide close to optimal convergence rate within the class and are appealing in practice due to their distributed nature.

In our setup, the gradient estimates supplied by the $K$ clients must pass through $r$-bit quantizers, %$Q_1, \ldots, Q_K$,
%\footnote{A quantizer $Q$ with input alphabet $\X$ and output alphabet $\Y$,
%  denoted $W\colon \X \to \Y$, represents
%  the conditional distribution of the output of
%  a randomized function given its input. In particular, $W(\cdot \mid x)$ is
%  the conditional distribution of the quantizer given that the input is $x\in \cX$.
%}
chosen 
%by the algorithm
from a fixed set of quantizers $\Q_r$\footnote{The set of $r$-bit quantizers $\Q_r$ is used to model the communication constraints in a distributed setting. }, and the optimization algorithm $\pi$ only has access to the quantized outputs.
%In particular, {for the $t$th query point $x_t$,  the gradient $\hat{g}_i(x_t)$ supplied by an client $O_i$ is passed through a quantizer.  
An \emph{$r$-bit quantizer} consists of randomized mappings $(Q^e, Q^d)$ with the encoder mapping ${Q^e:\R^d \to \{0,1\}^r}$ and the decoder mapping ${Q^d:\{0,1\}^r \to \R^d.}$ We denote the overall quantization procedure by the composition mapping $Q=Q^d\circ Q^e$. 
%which in turn can be viewed as the gradient processing quantizer $W_{i,t}$ for the client $O_i.$ Consequently, we express the corresponding quantizer output $Y_{i,t}$ as  $Q_i(\hat{g}_i(x_t)).$ After observing the outputs from all the clients, $\{Q_i(\hat{g}_i(x_t))\}_{i\in [K]}$ are passed through a mapping $Q: \R^{Kd}\to \R^d$ to give a $d$-dimensional vector used further for updating the query.

Our objective is to select quantizers $Q_{i,t}$, $\forall i \in [K], t \in [T],$ and an optimization algorithm $\pi$ to guarantee the minimum worst-case optimization error.  In our setting, we allow for {\em adaptive gradient processing,} whereby, the quantizer $Q_{i,t}$ selected in $t$th iteration may depend on all the previous quantized outputs. 
%$\{Q_{i, t^{\prime}}\}_{i\in [K], t^{\prime} \in [t-1]}$.
  Specifically, denoting by $Y_{i,t}$ the $i$th client's quantized output at time $t$,
%  which takes values in the output alphabet $\R^d,$
 the \emph{adaptive quantizer selection strategy} $S\eqdef (S_1, \ldots, S_T)$ over $T$ iterations 
consists of mappings $S_t\colon 
%\prod_{i \in [K], t^{\prime} \in [t-1]} 
\R^{dK(t-1)}\to \Q_r^K$ that take $\{Y_{i, t^{\prime}}\}_{i \in [K], t^{\prime} \in [t-1]}$ as input and outputs a tuple of $K$ quantizers ${\{Q_{i,t}\}_{i \in [K]}\in\Q_r^K}$.
We write $\mathcal{S}_{\Q_r, T}$ for the collection of all such quantizer selection strategies.
%{These quantized outputs $\{Y_{i,t}\}_{i\in [K]}$ are then used by the }
%At the end of $t$th iteration, the optimization algorithm $\pi$ updates the query point $x_t$ to $x_{t+1}$ using all the messages $\{Q_{i,t^\prime}(x_{t^\prime})\}_{i \in [K], t^{\prime} \in [t]}.$
The entire framework can be summarized as follows:
\begin{enumerate}
\item At iteration $t$, the first-order optimization algorithm $\pi$ makes a query for point $x_t$ to  clients $C_1, \ldots C_K$.
\item Upon receiving the point $x_t\in \X$, the client $i \in [K]$ outputs $\hat{g}_i(x_t)$, an unbiased estimate of  $\nabla f(x_t).$
%where $\E{\hat{g}_i(x_t)| x_t} = \nabla f (x_t)$ , $\forall i \in [K].$ 
\item The gradient estimate $\hat{g}_i(x_t)$ is passed through a quantizer $Q_{i,t} \in \Q_r$ chosen based on strategy $S$, and the output $Y_{i,t}$ is observed by the first-order optimization algorithm $\pi$. The algorithm then uses all the messages $\{Q_{i,t^\prime}(x_{t^\prime})\}_{i \in [K], t^{\prime} \in [t]}$ to further update $x_t$ to $x_{t+1}$.
\end{enumerate}
\noindent{Denote by $\clientset$ the collection of $K$ clients $(C_1, \ldots, C_K)$. Let $\Pi_T$ be the set of all first-order optimization algorithms that make $T$ queries to $\clientset$ and for the $t$th query $x_t$, get back the outputs $\{Y_{i,t}\}_{i \in [K]}$.
% with distribution $\{W_{i, t}(\cdot \mid \hat{g}_i(x_t))\}_{i \in [K]}$.}
We measure the performance of
an optimization protocol $\pi$ and a quantizer selection strategy $S$ for a given function $f$ and clients $C_i$, $i \in [K],$ using the metric
$\ep(f,  \clientset, \pi, S)$ defined as  \[\displaystyle{\hspace{1.5cm}
  \ep(f, \clientset, \pi, S) = \E{f\left(\bar{x}_T\right)-\min_{x\in \X} f(x)},}\]\\
%\end{equation} % C: either we put \eqdef for all three errors, or none; this one was the only one with \eqdef
where $\bar{x}_T:=\frac{1}{T}\sum_{t\in [T]}x_t$ and the expectation is over the randomness in $\bar{x}_T$.

For a set of various function and client pairs above, denoted by $\oO$, the set of $r$-bit quantizers $\mathcal{Q}_r$ and the number of iterations $T$, we define the \emph{minimax optimization error} as
\begin{align*}
%\label{eq:def:optimization:error}
  \ep^\ast(\X , \oO, T, \Q_r) =   \inf_{\pi \in \Pi_T}\inf_{S \in \mathcal{S}_{\Q_r, T}} \sup_{(f, \clientset)\in\oO}\ep(f, \clientset, \pi, S)\,.
\end{align*}
Below we will describe the class $\oO$ of interest to us.

\subsection{Function classes}
We now define the class of functions and state the assumptions related to the stochastic clients accessible to the algorithm $\pi$.
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Convex and smooth function family}
Throughout, we restrict
 ourselves to convex and $L$-smooth functions over $\X\subset\R^d$, i.e.,
functions  satisfying, $\forall \lambda \in [0, 1], \forall x, y \in \R^d$, 
 \begin{align} 
 f(\lambda x +(1-\lambda)y)&\leq \lambda f(x) +(1-\lambda)f(y), \quad \label{e:convexity}\\
\norm{\nabla f(x) - \nabla f(y)}_2 &\leq L \norm{x-y}_2,\label{e:L_smooth}
\end{align}
where $\nabla f(x)\in \R^d$ denotes the gradient of $f$ at input $x.$ 
%Further, the domain $\X$ has the diameter at most $D$, i.e., $\sup_{x,y\in \X} \|x-y\|\leq D$.
%\begin{align}
%\label{e:asmp_unbiasedness}
%\E{\hat{g}(x)\mid x} \in \partial f(x), \quad \text{(Unbiased estimates)} \\
%\label{e:asmp_as_bound}
%\bPr{\norm{\hat{g}(x)}_q^2 \leq B^2\mid x}=1, \quad \text{(Bounded estimates)}
%\end{align}

%at $x$ and $q\eqdef p/(p-1)$ is, \newer{as mentioned earlier,} the H\"older conjugate of $p$. We
%denote by $\oO_{{\tt c}, p}$ the set of all pairs of functions and clients satisfying Assumptions \eqref{e:convexity}, \eqref{e:asmp_unbiasedness}, and \eqref{e:asmp_as_bound}.



\paragraph{Stochastic gradients}
We assume that the output $\hat{g}_i(x)$ by client $C_i, 1\leq i\leq K,$ when a point $x\in \X$ is queried satisfies the following conditions:
\begin{align}\label{e:asmp_unbiasedness}
\E{\hat{g}_i(x)\mid x} &= \nabla f(x), \quad \text{(unbiased estimates)} \\
\label{e:varaince}
\norm{\hat{g}_i(x)-\nabla f(x)}_2^2 &\leq \sigma^2,\, \text{{(maximum deviation bound)}}
\\
\label{e:bounded_est}
\max_{x \in \X}\norm{\hat{g}_i(x)}_2^2 &\leq B^2.\qquad  \text{(a.s. bounded estimate)}
\end{align}


Assumption {\eqref{e:asmp_unbiasedness} is standard in stochastic optimization literature ($cf.$ \cite{nemirovsky1983problem}, \cite{nemirovski1995information}, \cite{bubeck2015convex}. However, it is enough to assume a bound on the variance of stochastic gradients instead of \eqref{e:varaince} to prove convergence guarantees for smooth stochastic optimization without any communication constraints. The stronger assumption made here is to aid a much tighter analysis under communication constraints. In Section \ref{s:extension}, we provide a scheme which can operate under the standard variance bound.}

Denote by $\oO_{\tt sc}$ the set of tuples of function and $K$ clients, $(f, \clientset)$, satisfying \eqref{e:convexity}, \eqref{e:L_smooth}, \eqref{e:asmp_unbiasedness}, \eqref{e:varaince} and \eqref{e:bounded_est}. 
\subsection{Lower bound}
Before proceeding further, the following bound will serve as a basic benchmark for our problem.
 Let $D>0$
and $\mathbb{X}_2(D) \eqdef \{\X \subseteq \R^d: \max_{x,y\in\X}\norm{x-y}_2\leq
D\}$ be the collection of subsets of $\R^d$ whose $\ell_2$ diameter is
at most $D$.

\begin{thm}\label{t:lb_smooth_coom_constraints}
  There exists an absolute constant $0\leq c_0\leq 1$ such that for $r  \in \N$ and $T \geq d/(6Kr),$
  %%% CC: We prove 9/58, so 1/6 (>9/58) works and is nicer.
\vspace{-5pt}
\[
 \sup_{\X \in \mathbb{X}_2(D)} \ep^*(\X , \oO_{{\tt sc}}, T, \Q_{r  }) 
\geq 
\frac{c_0D\sigma}{\sqrt{KT}} \cdot \sqrt{\frac{d}{d \wedge r}} .\]
\end{thm}
See Section \ref{p:lb} for proof. Note that affine function are $0$-smooth and admitted in the class of $L$ smooth functions. We use affine functions as difficult functions  and proceed in the same manner as in  the lower bounds for convex, Lipschitz optimization under  communication constraints (\cite[Section 4.5]{acharya2021nips};
see, also,~\cite{acharya2020general}), since the lower bounds for convex Lipschit optimization also use affine functions as difficult functions. 

%\begin{thm}\label{t:lb_smooth_priv_constraints}
% There exists an absolute constant $c_0>0$ such that, for $\varepsilon \in [0, 1]$, and $T \geq \frac{d}{k\epsilon^2},$ %%% CC: We prove 9/58, so 1/6 (>9/58) works and is nicer.
%\[
% \sup_{\X \in \mathbb{X}_2(D)} \ep^*(\X , \oO_{{\tt sc}}, T, \W_{{\tt priv}, \varepsilon }) 
%\geq 
%\frac{c_0D\sigma}{\sqrt{kT}} \cdot \sqrt{\frac{d}{\epsilon^2}} .\]
%\end{thm}
%\mnote{Removing the preivacy result}

\subsection{A general convergence bound}
We present a general convergence bound based on a non-adaptive channel strategy.  In particular,
we fix same quantization process in every iteration, and
% i.e., $Q_{i,t}=Q_i, \forall t\in [T]$, and
%Recall that the corresponding quantized output $Q_i(\hat{g}_i(x_t))$ is denoted by $Y_{i,t}.$ 
the quantized outputs $\{Y_{i,t}\}_{i\in [K]}$ are passed through a mapping ${Q: \R^{Kd}\to \R^d}$ in order to update the query.
%to give a $d$-dimensional vector used further for updating the query.
%\snote{The $\alpha, \beta$ parameters is a function of entire composition $Q\circ (Q_1, ...,Q_K)$, isn't it?.}

% $W_{1,t},...,W_{K,t}$,  the set of $K$ gradient processing quantizers chosen based on $S$ to give outputs $\{Y_{i,t}\}.$ Each output $Y_{i,t}$ can be 
%and by $\bar{Y}_t:=(Y_{1,t},..., Y_{k,t})$, the quantizer outputs after the $t$th query. Our proposed schemes involve projecting back these outputs in $\Pi_{i\in [K]}\Y_{i,t}$ to $\X$.
%In particular,  as a part of the optimization algorithm $\pi$, $\bar{Y}_t$ are passed through
%a mapping $Q: \Pi_{i\in [K],t^\prime\in t}\to \X$ which gives back a $d-$dimensional vector further used for updating the query.
%
%\snote{By enumeration 3.  in Page 3,\\
%1. The algorithm has $Y_{i,t}$s.  So, the decoding function W is assumed to be part of $\pi$.\\
%2.   if all the previous outputs are used,  $Q$ above becomes $Q_t$ to allow the size of variable inputs. In that case, the definitions of $\alpha, \beta$ below has to be changed accordingly too.}

We use PSGD as the first-order optimization algorithm; the overall optimization procedure is described in Algorithm \ref{a:SGD_Q}.  PSGD proceeds as SGD, with the additional projection step where it projects the updates back to domain $\X$ using the map $\Gamma_{\X}(y):=\min_{x\in \X}\|x-y\|$, $\forall\, y\in \R^d$. 

%\snote{The $\alpha, \beta$ parameters is a function of entire composition $Q\circ (Q_1, ...,Q_K)$, isn't it?.}

% $W_{1,t},...,W_{K,t}$,  the set of $K$ gradient processing quantizers chosen based on $S$ to give outputs $\{Y_{i,t}\}.$ Each output $Y_{i,t}$ can be 
%and by $\bar{Y}_t:=(Y_{1,t},..., Y_{k,t})$, the quantizer outputs after the $t$th query. Our proposed schemes involve projecting back these outputs in $\Pi_{i\in [K]}\Y_{i,t}$ to $\X$.
%In particular,  as a part of the optimization algorithm $\pi$, $\bar{Y}_t$ are passed through
%a mapping $Q: \Pi_{i\in [K],t^\prime\in t}\to \X$ which gives back a $d-$dimensional vector further used for updating the query.
%}
%\snote{By enumeration 3.  in Page 3,\\
%1. The algorithm has $Y_{i,t}$s.  So, the decoding function W is assumed to be part of $\pi$.\\
%2.   if all the previous outputs are used,  $Q$ above becomes $Q_t$ to allow the size of variable inputs. In that case, the definitions of $\alpha, \beta$ below has to be changed accordingly too.}

 \vspace{-0.1cm}
\begin{figure}[h]
 \vspace{-0.1cm}
\centering
\begin{tikzpicture}[scale=1, every node/.style={scale=1}]
\node[draw,text width= 6 cm , text height= ,] {%       
\begin{varwidth}{\linewidth}       
            \algrenewcommand\algorithmicindent{0.2em}
\begin{algorithmic}[1]
   \For{$t=0$ to $T-1$}
   %\State ~Observe $\bar{Y}_t=(Y_{1,t},...,Y_{K,t})$
	\State ~$x_{t+1}{=}\Gamma_{\X} \left(x_{t}-\eta_t Q(Y_{1,t},...,Y_{K,t})\right)$
   \EndFor \State Output $\bar{x}_T=\frac 1 T {\sum_{t=1}^T x_t}$
\end{algorithmic}
\end{varwidth}};
 \end{tikzpicture}
 \vspace{-0.1cm}
 \renewcommand{\figurename}{Algorithm}
\caption{PSGD with quantizers $\{Q_i\}_{i\in [K]}$}\label{a:SGD_Q}
\vspace{-0.1cm}
\end{figure}
%We now derive a convergence bound  described in Algorithm \ref{a:SGD_Q}. 
%In our formulation, the decoder $Q$ is a part of the optimization protocol $\pi$.
%As a result, the performance of the algorithm depends on both $Q$s and $S$s.
%For concreteness,
%with a slight abuse of notation 
%we now denote the overall optimization protocol using
%the tuple $(\pi, S, Q)$.
The convergence rate of Algorithm~\ref{a:SGD_Q} is controlled by the worst-case $L_2$-norm $\alpha(Q)$ and the worst-case bias $\beta(Q)$ defined as
\vspace{-0.25cm}
\begin{align}
&\alpha(Q):=\sup_{\substack{\{\forall x,i\in [K],\hat{g}_i \in \R^d:\\ {\|\hat{g}_i-\nabla f(x)\|^2}\leq \sigma^2\}}} \sqrt{\E {\| Q(\bar{Y})-\nabla f(x)\|^2}}, \label{def_a}\\
&\beta(Q):=\sup_{\substack{\{\forall x,i\in [K],\hat{g}_i \in \R^d:\\ {\|\hat{g}_i-\nabla f(x)\|^2}\leq \sigma^2\}}}\|\E {(Q(\bar{Y})-\nabla f(x)}\|, \label{def_b}
\vspace{-0.25cm}
\end{align}
where for $i\in [K], \bar{Y}=(Y_{1,t},...,Y_{K,t}).$
{Using a slight  modification of the standard proof of convergence for PSGD, we can derive the following lemma.}
%is the quantized output of $i$th client based on the strategy described above.
%The next result is only a minor modification of the standard PSGD proof and is very similar to  \cite[Theorem \textcolor{red1}{2.4}]{mayekar2020ratq}.
\begin{lem}\label{l:general}
For any mapping $Q$ and set of quantizers $\{Q_i\}_{i\in [K]}$ defined above, the output $\bar{x}_T$ of optimization algorithm given in Algorithm \ref{a:SGD_Q} satisfies
\begin{align*}
&\sup_{(f,\clientset)\in \cO}\cE(f, \clientset, \pi, S) \\
&\quad\leq \frac{\sqrt{2}\alpha(Q)D}{\sqrt{T}}+\beta(Q)\left(D+\frac{DB}{\alpha(Q)\sqrt{2T}}\right)+\frac{LD^2}{2T},
\end{align*}
with the learning rate $\eta_t=
\min\{\frac{1}{L}, \frac{D}{\alpha(Q)\sqrt{2T}}\}, \forall t\in [T.]$ 
%for all iterations $t \in [T]$.
\label{thm1} 
\end{lem}

\subsection{Sub-gaussian norm and random rotation}
For our analysis, it will be convenient to recall the definition of subgaussian norm\footnote{$\norm{\cdot}_{\psi_2}$ is indeed a norm.} of a random variable. %the subexponential norm of a random variable.
\begin{defn}[{\cite[Def. 2.5.6]{vershynin2018high}}]
A subgaussian norm of a subgaussian random variable $X$, denoted $\norm{X}_{\psi_2},$ is defined as $\norm{X}_{\psi_2} := \inf\{t>0: \E{e^{X^2/t^2}}\leq 2  \}.$ It follows that for a centered subgaussian random variable $X,$ 
$\Pr(|X|)\geq t) \leq 2 e^{-\frac{t^2 }{\norm{X}_{\psi_2}^2}}.$
\end{defn}
\begin{defn}[{\cite[Def. 2.7.5]{vershynin2018high}}]
A subexponential norm of a  subexponential random variable $X$, denoted $\norm{X}_{\psi_1},$ is defined as $\norm{X}_{\psi_1} := \inf\{t>0: \E{e^{\frac{|X|}{t}}}\leq 2  \}.$ It follows that for a centered subexponential  random variable $X,$ $\Pr(|X|)\geq t) \leq 2 e^{-\frac{t }{\norm{X}_{\psi_1}}}.$
\end{defn}
In addition to this, we require a random Hadamard matrix to perform random rotation.
Specifically, denoting by ${H}$ the $d\times d$ Walsh-Hadamard Matrix (See \cite{horadam2012hadamard}), define 
\begin{align}\label{e:rotation}
{R}:=1/\sqrt{d}{H}D^\prime,
\end{align}
 where $D^\prime$ is a diagonal matrix with each diagonal entry generated  uniformly from $\{-1,+1\}.$


